Engineering Reliable Interactions in the Reality-Artificiality Continuum

Milgram's reality-virtuality continuum applies to interaction in the physical space dimension, going from real to virtual. However, interaction has a social dimension as well, that can go from real to artificial depending on the companion with whom the user interacts. In this paper we present our vision of the Reality-Artificiality bidimensional Continuum (RAC), we identify some challenges in its design and development and we discuss how reliable interactions might be supported inside RAC.

==> eptcsdata.tex <==
\providecommand{\firstpage}{69}
\providecommand{\publicationstatus}{R.C. Cardoso, A. Ferrando, D. Briola, C. Menghi,\\ T. Ahlbrecht (Eds.): First Workshop on Agents and\\ Robots for reliable Engineered Autonomy 2020 (AREA'20).\\
EPTCS 319, 2020, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.319.6}{10.4204/EPTCS.319.6}}
\pdfoutput=1

